RainyGS: Efficient Rain Synthesis with Physically-Based Gaussian Splatting

We consider the problem of adding dynamic rain effects to in-the-wild scenes in a physically-correct manner. Recent advances in scene modeling have made significant progress, with NeRF and 3DGS techniques emerging as powerful tools for reconstructing complex scenes. However, while effective for novel view synthesis, these methods typically struggle with challenging scene editing tasks, such as physics-based rain simulation. In contrast, traditional physics-based simulations can generate realistic rain effects, such as raindrops and splashes, but they often rely on skilled artists to carefully set up high-fidelity scenes. This process lacks flexibility and scalability, limiting its applicability to broader, open-world environments. In this work, we introduce RainyGS, a novel approach that leverages the strengths of both physics-based modeling and 3DGS to generate photorealistic, dynamic rain effects in open-world scenes with physical accuracy. At the core of our method is the integration of physically-based raindrop and shallow water simulation techniques within the fast 3DGS rendering framework, enabling realistic and efficient simulations of raindrop behavior, splashes, and reflections. Our method supports synthesizing rain effects at over 30 fps, offering users flexible control over rain intensity -- from light drizzles to heavy downpours. We demonstrate that RainyGS performs effectively for both real-world outdoor scenes and large-scale driving scenarios, delivering more photorealistic and physically-accurate rain effects compared to state-of-the-art methods. Project page can be found at https://pku-vcl-geometry.github.io/RainyGS/

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}



\begin{figure*}
	\centering
	\setlength{\tabcolsep}{1pt}
	\setlength{\imagewidth}{0.19\textwidth}
	\begin{tabular}{m{0.38cm}<{\centering}m{\imagewidth}<{\centering}m{\imagewidth}<{\centering}m{\imagewidth}<{\centering}m{\imagewidth}<{\centering}m{\imagewidth}<{\centering}}
		& $t=\SI{3}{\second}$ & $t=\SI{6}{\second}$ & $t=\SI{9}{\second}$ & $t=\SI{12}{\second}$ & $t=\SI{15}{\second}$\\
		\rotatebox{90}{\textbf{2D Processing}} &
		\includegraphics[width=\imagewidth]{img/fixed_view/2d/rain_1.jpg} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/2d/rain_11.jpg} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/2d/rain_21.jpg} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/2d/rain_31.jpg} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/2d/rain_41.jpg}\\
		\rotatebox{90}{\textbf{Video Diffusion}} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/aigv/frame_0000.jpg} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/aigv/frame_0006.jpg} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/aigv/frame_0012.jpg} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/aigv/frame_0018.jpg} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/aigv/frame_0024.jpg}\\
		\rotatebox{90}{\textbf{Ours}} &
		\includegraphics[width=\imagewidth]{img/fixed_view/ours/0010.png} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/ours/0020.png} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/ours/0030.png} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/ours/0040.png} & 
		\includegraphics[width=\imagewidth]{img/fixed_view/ours/0050.png}\\
	\end{tabular}
	\caption{\label{fig:fixed_view}Qualitative Results. WE NEED TO SHOW ZOOM-IN VIEWS}
\end{figure*}

\begin{comment}

	In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured in the sunnmy or cloudy weather conditions, synthesizing its correspiding rainy conditions in a photorealistc and physically-correct manner. 
	%
	The rain syntheis for arbitrary open scenes plays an important role in a wild range of applications, inlcuding AR/VR, gaming, robotics and more~\cite{}. 
	%
	However, it is also extrememly challening, as realisitc rainy effcts inlcuidng various high-order physics and rendering effects such as the  rain lines in the sky, the water on the ground, the reflection and refractions rendering effects.  More importantly, these apsects reuqires dynamic modeling, \ie, all of them should apprear in the same time and dynmaiclly, making it a chaleelinging problme that still under explored.
	
	In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize corresponding rainy conditions in a photorealistic and physically-correct manner.
	%
	Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and more~\cite{}.
	%
	However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physics and rendering phenomena. For example, these include the formation of rain streaks in the sky, the accumulation of water on the ground, and realistic reflection and refraction effects.
	%
	More importantly, these elements require occur concurrenctly and evolve dynamiclly over time, further adding its diffculities and making this problem remains largely underexplored.
	
	\
	In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize its corresponding rainy conditions in a photorealistic and physically-accurate manner.
	%
	Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and more~\cite{}.
	%
	However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physical and rendering phenomena. For instance, this includes the formation of rain streaks in the sky, the accumulation of water on the ground, and realistic reflection and refraction effects.
	%
	Moreover, these elements must appear concurrently, evolve dynamically over time, and can be simulated in an efficient way to statify the requirements of a border applicating, which further adds the complexity and making this problem largely underexplored.
	
	
\end{comment}





In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize its corresponding rainy conditions in a photorealistic and physically-accurate manner.
%
Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and more~\cite{}. For example, it allows people using AR glasses to imaging xxx , it also helps embodied robots and autodriving carts to be trained on more challenging weather conditions to increase the saftely and reliability.
%
However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physical and rendering phenomena. This includes the formation of rain streaks in the sky, the accumulation of water on the ground, and realistic reflection and refraction effects.
%
Moreover, these elements must appear concurrently, evolve dynamically over time, and be simulated efficiently to meet the demands of broader applications---further increasing the complexity and making this problem largely underexplored.




In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize its corresponding rainy conditions in a photorealistic and physically-accurate manner.

Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and autonomous driving~\cite{}. For example, it not only enables AR glasses experiencing realistic rain effects in virtual outdoor environments, enriching applications in entertainment and travelling, but also allows embodied robots and autonomous vehicles to be trained in challenging rainy conditions, enhancing their safety and reliability.
%
However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physical and rendering phenomena. This includes the formation of rain streaks in the sky, the accumulation of water on the ground, and realistic reflection and refraction effects.
%
Moreover, these elements must appear concurrently, evolve dynamically over time, and be simulated efficiently to meet the demands of broader applications---further increasing the complexity and making this problem largely underexplored.


In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize its corresponding rainy conditions in a photorealistic and physically-accurate manner.
%
Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and autonomous driving~\cite{}. 
%
For example, it not only enables AR glasses to display realistic rain effects in virtual outdoor environments, enriching applications in entertainment and travel, but also allows embodied robots and autonomous vehicles to be trained in challenging rainy conditions, enhancing their safety and reliability.

However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physical and rendering phenomena. This includes the formation of rain streaks in the sky, water accumulation on surfaces, and realistic reflection and refraction effects.

Furthermore, these elements must appear concurrently, evolve dynamically over time, and be simulated efficiently to meet the demands of broader applications—further increasing complexity and making this problem largely underexplored.



%###

This paper presents RainyGS, a high-fidelity and interactive rain simulator that integrates 3D-GS-based scene representation, shallow-water dynamics, and screen-space ray tracing. Each component is thoughtfully integrated as an ideal fit to achieve visual realism, physical accuracy, and computational efficiency for complex, in-the-wild rainy scenarios. Our contributions include: 1) adapting shallow-water dynamics to 3D GS scenes for its real-time performance and high-fidelity rainy phenomena, effectively capturing water wave and ripple effects for visual realism while providing better physical accuracy than position-based dynamics, 2) employing screen-space ray tracing to enhance the visual fidelity of Gaussian splatting by capturing high-quality reflections and refractions, which aligns with rasterization pipelines and supports efficient rendering, and 3) in together delivering an interactive simulation tool that supports high-fidelity rain with complete 3D and time annotations and physically precise user interactions, serving as valuable augmentation for data in downstream applications. Compared to existing video-based methods, RainyGS maintains 3D consistency and physical correctness, with substantial potential for even further optimization and broader applicability.



==> sec/1_intro_v2.tex <==
\section{Introduction}
\label{sec:intro}


\begin{comment}

	In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured in the sunnmy or cloudy weather conditions, synthesizing its correspiding rainy conditions in a photorealistc and physically-correct manner. 
	%
	The rain syntheis for arbitrary open scenes plays an important role in a wild range of applications, inlcuding AR/VR, gaming, robotics and more~\cite{}. 
	%
	However, it is also extrememly challening, as realisitc rainy effcts inlcuidng various high-order physics and rendering effects such as the  rain lines in the sky, the water on the ground, the reflection and refractions rendering effects.  More importantly, these apsects reuqires dynamic modeling, \ie, all of them should apprear in the same time and dynmaiclly, making it a chaleelinging problme that still under explored.
	
	In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize corresponding rainy conditions in a photorealistic and physically-correct manner.
	%
	Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and more~\cite{}.
	%
	However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physics and rendering phenomena. For example, these include the formation of rain streaks in the sky, the accumulation of water on the ground, and realistic reflection and refraction effects.
	%
	More importantly, these elements require occur concurrenctly and evolve dynamiclly over time, further adding its diffculities and making this problem remains largely underexplored.
	
	\
	In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize its corresponding rainy conditions in a photorealistic and physically-accurate manner.
	%
	Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and more~\cite{}.
	%
	However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physical and rendering phenomena. For instance, this includes the formation of rain streaks in the sky, the accumulation of water on the ground, and realistic reflection and refraction effects.
	%
	Moreover, these elements must appear concurrently, evolve dynamically over time, and can be simulated in an efficient way to statify the requirements of a border applicating, which further adds the complexity and making this problem largely underexplored.
	
	
	
	In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize its corresponding rainy conditions in a photorealistic and physically-accurate manner.
	%
	Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and more~\cite{}. For example, it allows people using AR glasses to imaging xxx , it also helps embodied robots and autodriving carts to be trained on more challenging weather conditions to increase the saftely and reliability.
	%
	However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physical and rendering phenomena. This includes the formation of rain streaks in the sky, the accumulation of water on the ground, and realistic reflection and refraction effects.
	%
	Moreover, these elements must appear concurrently, evolve dynamically over time, and be simulated efficiently to meet the demands of broader applications---further increasing the complexity and making this problem largely underexplored.
	
	
	
	
	In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize its corresponding rainy conditions in a photorealistic and physically-accurate manner.
	
	Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and autonomous driving~\cite{}. For example, it not only enables AR glasses experiencing realistic rain effects in virtual outdoor environments, enriching applications in entertainment and travelling, but also allows embodied robots and autonomous vehicles to be trained in challenging rainy conditions, enhancing their safety and reliability.
	%
	However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physical and rendering phenomena. This includes the formation of rain streaks in the sky, the accumulation of water on the ground, and realistic reflection and refraction effects.
	%
	Moreover, these elements must appear concurrently, evolve dynamically over time, and be simulated efficiently to meet the demands of broader applications---further increasing the complexity and making this problem largely underexplored.
	
	
\end{comment}


In this paper, we investigate how to add photorealistic rain effects to in-the-wild scenes, \ie, given multi-view images of an open-world scene captured under sunny or cloudy conditions, we aim to synthesize its corresponding rainy conditions in a photorealistic and physically-accurate manner.
%
Rain synthesis for open-world scenes plays a critical role in a wide range of applications, including AR/VR, gaming, robotics, and autonomous driving~\cite{}. 
%
For example, it not only enables AR glasses to display realistic rain effects in virtual outdoor environments, enriching applications in entertainment and travel, but also allows embodied robots and autonomous vehicles to be trained in challenging rainy conditions, enhancing their safety and reliability.
%
However, achieving realistic rain effects is highly challenging, as it involves simulating complex, high-order physical and rendering phenomena. This includes the formation of rain streaks in the sky, water accumulation on surfaces, and realistic reflection and refraction effects.
%
Furthermore, these elements must appear concurrently, evolve dynamically over time, and be simulated efficiently to meet the demands of broader applications---further increasing complexity and making this problem largely underexplored.


\begin{comment}
	
	The rain synthesis problem is closely related to two important research domians:  scene modelling and physics-based simulations.  Recnetly, 3D scene modeling has witnessed great progress, with the raipdly growding of advanced neural radiance (NeRF) and 3D Gaussian Splatting (3DGS). Those methods further evolved beyond novel view synthesis but also extend to advanced scene edititing. However, most of existing wortks focus on inverse rendering and primary editing the scene's lighitng condition, still fall begind more advanced, pysically based editing tasks such as rain simulation.
	%
	Althernatively, physics-based simulations apply physicas rule to synthesize realistic rain effects, like raindrops and splashes, but they generally rely on skilled artists to carefully set up high-fidelity scenes. This process lacks flexibility and diversity, limiting its scope for broader applications.
	%
	Rencetly, ClimateNeRF and Gaussian Splahing pionnered in combining Neural Fields r 3DGS and physicals simulation to syntheize hash waeaks or fluid effects and ahivene impressieve eddtin results. However, these focus on static modeling and requires slow simulation efects, which can hardly be extended to realisic rain thesis and lack the required efficiency for for broader applications.
	
	
	The in-the-wild rain synthesis problem is closely related to two important research domains: scene modeling and physics-based simulations. 
	%
	Nowadays, 3D scene modeling has made significant progress. 
	%
	Neural Radiance Fields (NeRF) and 3D Gaussian Splatting (3DGS)~\cite{bibid} techniques have emerged as powerful tools not only advancing novel view synthesis but also extended to more complex tasks such as scene editing. 
	%
	However, most existing works focus primarily on inverse rendering-based illumination editing tasks, but still fall short of more advanced, physics-based editing tasks like rain simulation.
	%
	Alternatively, physics-based simulations use physical principles to generate realistic rain effects, such as raindrops and splashes. However, these methods often rely on skilled artists to manually set up high-fidelity scenes, which lacks flexibility and diversity, limiting its applicability to in-the-wild contexts.
	%
	Very recently, ClimateNeRF~\cite{bibid} and Gaussian Splashing~\cite{Splatting} have pioneered the integration of scene modeling and physics-based simulations to synthesize extreme weather or fluid effects, achieving impressive editing results. 
	%
	However, the former primarily focus on static weather modeling while the latter utilizes ineficient partical  simulations, making them unsuitable for dynamic rain synthesis and lacking the necessary efficiency for broader applications.
	
	
\end{comment}



The problem of in-the-wild rain synthesis is closely related to two important research domains: scene modeling and physics-based simulations.
% 
In recent years, 3D scene modeling has made significant progress: techniques such as Neural Radiance Fields (NeRF) and 3D {\gs} ({\gsshort})~\cite{bibid} have emerged as powerful tools, not only advancing novel view synthesis but also enabling more complex tasks like scene editing. 
%
However, most existing works~\cite{bibid} focus primarily on inverse rendering-based illumination editing, falling short of more advanced, physics-based editing tasks such as rain simulation.
%
Alternatively, physics-based simulations use physical principles to generate realistic rain effects, including raindrops and splashes. These methods, however, often rely on skilled artists to manually set up high-fidelity scenes, which limits their flexibility and applicability for in-the-wild contexts.
%
Recently, ClimateNeRF~\cite{bibid} and Gaussian Splashing~\cite{Splatting} have pioneered the integration of scene modeling and physics-based simulations to synthesize extreme weather or fluid effects, achieving impressive editing results. Nevertheless, the former focuses mainly on static weather modeling, % with  volumetric ray tracing, 
while the latter employs inaccurate particle simulations,
% particle simulation is efficient, but not accurate for rain
making both approaches unsuitable for efficient and dynamic rain synthesis. % and lacking the efficiency required for broader applications.

\begin{comment}
	
	To fill this gap, we propose {\name}, a physically-based 3D Gaussian Splatting  simulation framework that enables  effecient and photo-realisitc rain synthesis for in-the-wild scenes. 
	%
	{\name} leverages the strength of accurate physics-based rain simulation methods as well as efficient Gaussian Splatting Rendering framework, achving physically-accurate and fast rain simulation results.
	%
	Specifically, given multi-view images as input, we first apply 3DGS to model the scene and disentangle the corresponding geometry material, and illumination conditions. 
	%
	We then apply physics modelsing appraoches to add realsict rain effects, including the flying rain streaks, accumulated rain woater on the rgroud, and high-order effects such as relfection, reflections and specular rendering effects.
	%
	We carefully choose proper and efficient simulation techniques, utlizing shock wave to model the surface water and xxxx to model reflections.  
	% 
	Consequenclty, it supports precisely model all the necessary rainy effects like drops, water on the ground, splashes, reflection  jointly, providing free-view photorealisic modeling results for open-world scenes.
\end{comment}

To fill this gap, we propose {\name}, a physics-based 3D Gaussian Splatting simulation framework that enables efficient and photorealistic rain synthesis for in-the-wild scenes.
%
{\name} combines the accuracy of physics-based rain simulation methods with the efficiency of the {\gs} rendering framework, achieving both physically accurate and fast rain simulation results.
%
Specifically, given multi-view images as input, we first use 3DGS to model the scene and disentangle its corresponding geometry, material, and illumination conditions.
% 
Next, we apply physics-based models to add realistic rain effects, including flying rain streaks, accumulated water on the ground, and high-order effects such as reflections, refractions, and specular rendering.
%
\cmy{
This is challenging due to Gaussian's limitation on lacking accurate geometry and its unsuitability for rendering reflections, owing to its splatting technology.
%
Our approach addresses these challenges by thoughtfully integrating high-fidelity and efficient simulation and rendering techniques.
For the dynamics, we adapt shallow-water simulation \cite{chentanez2010real}, whose physical assumptions are particularly well-suited for rain scenarios and provide more accurate results than position-based dynamics. Utilizing height fields to model surface water dynamics not only circumvents the geometric limitations of GS but also ensures real-time efficiency.
For rendering, we integrate screen-space ray tracing \cite{mcguire2014ray} with 3D GS to accurately render reflections of visible parts, which are most critical to visual experience and well-suited for rasterization pipelines.
}
% I feel it is important to explain why integrating shallow water and screen-space rendering is not a simple A+B, but a perfect fit for RainyGS
Consequently, {\name} enables precise modeling of all necessary rainy effects—such as raindrops, water on the ground, splashes, and reflections—providing photorealistic, free-view rain thesis for in-the-wild scenes.


{\name} provides a unified, open-world rain synthesis framework, enabling efficient and realistic rain effects with physical accuracy.
%
Notably, it renders rain effects at a fast speed of more than 10 fps and allows users to freely control rain intensity, from light drizzle to heavy downpour (c-e), achieving high-quality, realistic results in a computationally efficient manner.
%
We validate our method across diverse in-the-wild scenes, including tank and template datasets, MipNeRF scenes, and Waymo driving scenarios, demonstrating superior simulation performance, high-fidelity preservation, and better user control compared to 2D-based editing methods and video generation baselines.
% 
In summary, our contributions include:

\begin{itemize}
 

\item  adapting shallow-water dynamics to 3D GS scenes for its real-time performance and high-fidelity rainy phenomena, effectively capturing water wave and ripple effects for visual realism while providing better physical accuracy than position-based dynamics,
\item  employing screen-space ray tracing to enhance the visual fidelity of Gaussian splatting by capturing high-quality reflections and refractions, which aligns with rasterization pipelines and supports efficient rendering, and 
\item  in together delivering an interactive simulation tool that supports high-fidelity rain with complete 3D and time annotations and physically precise user interactions, serving as valuable augmentation for data in downstream applications. 

\end{itemize}

% we presents RainyGS, a high-fidelity and interactive rain simulator that integrates 3D-GS-based scene representation, shallow-water dynamics, and screen-space ray tracing. Each component is thoughtfully integrated as an ideal fit to achieve visual realism, physical accuracy, and computational efficiency for complex, in-the-wild rainy scenarios. Our contributions include: 1) adapting shallow-water dynamics to 3D GS scenes for its real-time performance and high-fidelity rainy phenomena, effectively capturing water wave and ripple effects for visual realism while providing better physical accuracy than position-based dynamics, 2) employing screen-space ray tracing to enhance the visual fidelity of Gaussian splatting by capturing high-quality reflections and refractions, which aligns with rasterization pipelines and supports efficient rendering, and 3) in together delivering an interactive simulation tool that supports high-fidelity rain with complete 3D and time annotations and physically precise user interactions, serving as valuable augmentation for data in downstream applications. Compared to existing video-based methods, RainyGS maintains 3D consistency and physical correctness, with substantial potential for even further optimization and broader applicability.


==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\begin{figure*}
	\centering
	\includegraphics[width=1\linewidth,height=6cm]{example-image}
	\caption{\label{fig:pipeline}Method illustration. This figure provides an overview of our pipeline.}
\end{figure*}


In this section, we review three related topics. 
We first talk about recent scene modeling and editing achievements.
% novel view synthesis (NVS) methods based on physically-based rendering. 
Next, we describe physically-based weather simulation works. 
%
Lastly, we discuss physically-based Gaussian Spllating modeling and editing works. % 3D scene editing that utilizes Radiance Fields.

\paragraph{Physically-Based Rendering for NVS}
% nerf: Nerd, Neural-pil, TensoIR, Sire-ir, Neilf++, Nerfactor, physg
% 3dgs: gaussianshader, gir, r3gs, gs-ir, (3dgs-dr, GS^3)
%\xy{Talk about specular reflection}
NVS aims to generate the appearance of a 3D scene from new camera poses using a set of images captured from discrete viewpoints. 
Neural Radiance Fields (NeRF)~\cite{mildenhall2020nerf} encode the plenoptic function and volume density into a Multi-Layer Perceptron (MLP), enabling realistic view synthesis through volume rendering.
Recently, 3D Gaussian Splatting (3DGS)~\cite{kerbl20233d} has emerged as an advanced NVS approach, offering real-time, high-quality rendering by representing scenes as collections of 3D Gaussian ellipsoids and utilizing fast rasterization.
However, such representations inherently entangle geometry, material, and lighting, making scene editing challenging. To mitigate this, several NeRF-based methods [] incorporate Physically-Based Rendering (PBR) to decouple the scene into material and lighting attributes. 
NeRD~\cite{boss2021nerd} is the first to extend NeRF by utilizing the MLP to parameterize the BRDF field.


physg, TensoIR

gs-ir,r3gs, gaussianshader


\paragraph{Realistic Weather Synthesis}
\xy{The importance of making climate simulations accessible is well known. [66] collects climate images dataset and performs image editing with CycleGAN[98]. [18, 67] leverage depth information to estimate water mask, and perform GAN-based image editing and inpainting. [29] simulate fog and snow. These methods offer realistic effects for a single image, but cannot provide immersive, view-consistent climate simulation. In contrast, ClimateGAN allows the view to move without artifacts.
Physically-based simulation of weather: Physical simulation of weather in computer graphics has too long a history to allow comprehensive review here. Fournier and Reeves obtain excellent capillary wave simulations with
simple Fourier transform reasoning [23] (and we adopt their method), with modifications by [31, 78];[21] simulates smoke; and [57, 22, 71] simulate snow in wind using metaballs and fluid dynamics. Our method demonstrates how to benefit from such simulations while retaining the excellent scene modelling properties of NeRF style models}

\paragraph{Radiance Field Editing}
%Gaussian Splatting Editing
%climatenerf, gaussiansplashing
%\xy{Can NeRF papers be here? Is `Dynamic Neural Radiance Fields' more accurate?}
\qy{Gaussian splatting editing is an emerging approach in novel view synthesis that leverages Gaussian primitives to represent scenes in a compact and efficient manner. Unlike traditional mesh-based or voxel-based representations, Gaussian splatting uses 2D Gaussian distributions projected into 3D space to model scene geometry and appearance. This approach has advantages in terms of memory efficiency and rendering speed, making it suitable for real-time applications. Gaussian splatting allows for intuitive manipulation of scene content by editing the parameters of the Gaussian primitives, such as their position, scale, and color attributes. Recent methods focus on optimizing these parameters using differentiable rendering techniques, enabling interactive scene editing and view synthesis with minimal artifacts. These methods have been extended to handle dynamic scenes by incorporating temporal consistency constraints, ensuring that the edited Gaussian parameters remain coherent across frames. However, challenges include managing the complexity of scenes with a high number of Gaussian primitives and ensuring accurate occlusion handling, especially in scenarios with dense object overlaps or intricate structures.}




==> src_sup/derivatives.tex <==
\section{Derivatives of the Elastic Energy}
\label{apx:derivative}

We bypass the medium of deformation gradients and compute the first- and second-order partial derivatives of $V_\mathrm{e}$ w.r.t. nodal degrees of freedom $\{\bm{q}_I\}$ directly.

\subsection{The First-Order Derivatives (Force)}

With the total elastic potential energy defined by $V_\mathrm{e}=\iint_{\bar{\Omega}}\bar{\mathcal{V}_\mathrm{e}}\,\mathrm{d}\bar{\Omega}$,
according to Eq.~(11) in the main text, the first-order partial derivatives of the elastic energy are given by
\begin{align}
  \frac{\partial V_\mathrm{e}}{\partial \bm{q}_I}
  =&\iint_{\bar{\Omega}}\frac{\partial\bar{\mathcal{V}}_\mathrm{e}}{\partial\bm{q}_I}\,\mathrm{d}\bar{\Omega}\notag\\
  =&\iint_{\omega}\frac{\partial\bar{\mathcal{V}}_\mathrm{e}}{\partial\bm{q}_I}\sqrt{\bar{a}}\,\mathrm{d}\xi^1\mathrm{d}\xi^2\notag\\
  =&\iint_{\omega}\left(\tau\frac{\partial a_{\alpha\beta}}{\partial\bm{q}_I}A_{\gamma\delta}+\frac{1}{3}\tau^3\frac{\partial b_{\alpha\beta}}{\partial\bm{q}_I}B_{\gamma\delta}\right)\bar{H}^{\alpha\beta\gamma\delta}\sqrt{\bar{a}}\,\mathrm{d}\xi^1\mathrm{d}\xi^2\text{,}\label{eqn:intdeltave}
\end{align}
with partial derivatives of $a_{\alpha\beta}$ and $b_{\alpha\beta}$ are calculated by
\begin{align}
   \label{eqn:paabpqi}
      \frac{\partial a_{\alpha\beta}}{\partial \bm{q}_I}= &\varPhi^I_{,\alpha}\bm{a}_\beta+\varPhi^I_{,\beta}\bm{a}_\alpha\text{,}\\
      \label{eqn:pbabpqi}
      \frac{\partial b_{\alpha\beta}}{\partial \bm{q}_I}= &\varPhi^I_{,\alpha\beta}\bm{a}_3+\frac{1}{\sqrt{a}}\left(\varPhi^I_{,1}\bm{a}_2\times\bm{a}_{\alpha,\beta}+\varPhi^I_{,2}\bm{a}_{\alpha,\beta}\times\bm{a}_1\right. \notag\\ 
       &-\left.\bm{a}_{\alpha,\beta}\cdot\bm{a}_3(\varPhi^I_{,1}\bm{a}_2\times\bm{a}_3+\varPhi^I_{,2}\bm{a}_3\times\bm{a}_1)\right)\text{.}
\end{align}

In order to facilitate numerical calculation, we rewrite Eq.~(\ref{eqn:intdeltave}) in a matrix form using \emph{Voigt notation} as
\begin{equation}
  \label{eqn:matrix}
  \frac{\partial V_\mathrm{e}}{\partial \bm{q}_I}=
  \iint_{\omega}\left(\tau\left(\frac{\partial\bm{\alpha}}{\partial\bm{q}_I}\right)^\mathrm{T}\bm{H}\bm{\alpha}+\frac{1}{12}\tau^3\left(\frac{\partial\bm{\beta}}{\partial\bm{q}_I}\right)^\mathrm{T}\bm{H}\bm{\beta}\right)\sqrt{\bar{a}}\,\mathrm{d}\xi^1\mathrm{d}\xi^2\text{,}
\end{equation}
where $\bm{H}=(H^{ij})_{3\times3}$ is a square matrix, and $\bm{\alpha}=(\alpha_i)_{3\times1}$ and $\bm{\beta}=(\beta_i)_{3\times1}$ are column vectors.
It should be noted that a mixed layout is used here --- first-order partial derivatives are always written as column vectors. Considering the symmetry of the quantities, the matrix and vectors in this integral can be written as
\begin{gather}
  \bm{H}=
  {\small\begin{pmatrix}
    (\lambda+2\mu)(\bar{a}^{11})^2 & \lambda\bar{a}^{11}\bar{a}^{22}+2\mu(\bar{a}^{12})^2 & (\lambda+2\mu)\bar{a}^{11}\bar{a}^{12}\\
    & (\lambda+2\mu)(\bar{a}^{22})^2 & (\lambda+2\mu)\bar{a}^{12}\bar{a}^{22}\\
    \text{sym.} & & (\lambda+\mu)(\bar{a}^{12})^2+\mu\bar{a}^{11}\bar{a}^{22}
  \end{pmatrix}}%
  \text{,}\\
  \bm{\alpha}=
  \begin{pmatrix}
    A_{11} & A_{22} & 2A_{12}
  \end{pmatrix}^\mathrm{T}
  \text{,}\\
  \bm{\beta}=2
  \begin{pmatrix}
    B_{11} & B_{22}& 2B_{12}
  \end{pmatrix}^\mathrm{T}
  \text{,}\\
  \frac{\partial\bm{\alpha}}{\partial\bm{q}_I}=
  \frac{1}{2}
  \begin{pmatrix}
    \frac{\partial a_{11}}{\partial \bm{q}_I}
    & \frac{\partial a_{22}}{\partial \bm{q}_I}
    & 2\frac{\partial a_{12}}{\partial \bm{q}_I}
  \end{pmatrix}^\mathrm{T}
  \text{,}\\
  \frac{\partial\bm{\beta}}{\partial\bm{q}_I}=
  \begin{pmatrix}
    \frac{\partial b_{11}}{\partial \bm{q}_I}
    & \frac{\partial b_{22}}{\partial \bm{q}_I}
    & 2\frac{\partial b_{12}}{\partial \bm{q}_I}
  \end{pmatrix}^\mathrm{T}
  \text{.}
\end{gather}

\subsection{The Second-Order Derivatives (Hessian)}

The Hessian matrix is given by
\begin{align}
    \frac{\partial^2V_\mathrm{e}}{\partial\bm{q}_J\partial\bm{q}_I}&=\iint_{\bar{\Omega}}\frac{\partial^2\bar{\mathcal{V}}_\mathrm{e}}{\partial\bm{q}_J\partial\bm{q}_I}\,\mathrm{d}\bar{\Omega}\notag\\
  &=\iint_{\omega}\left(\tau\,\bm{G}_1+\frac{1}{12}\tau^3\,\bm{G}_2\right)\sqrt{\bar{a}}\,\mathrm{d}\xi^1\mathrm{d}\xi^2\text{,}
\end{align}
in which the following equations hold:
\begin{align}
  \bm{G}_1&=\left(\frac{\partial\bm{\alpha}}{\partial\bm{q}_I}\right)^\mathrm{T}\bm{H}\left(\frac{\partial\bm{\alpha}}{\partial\bm{q}_J}\right)+\sum_{i=1}^3\sum_{j=1}^3\frac{\partial^2\alpha_i}{\partial\bm{q}_J\partial\bm{q}_I}H^{ij}\alpha_j\text{,}\\
  \bm{G}_2&=\left(\frac{\partial\bm{\beta}}{\partial\bm{q}_I}\right)^\mathrm{T}\bm{H}\left(\frac{\partial\bm{\beta}}{\partial\bm{q}_J}\right)+\sum_{i=1}^3\sum_{j=1}^3\frac{\partial^2\beta_i}{\partial\bm{q}_J\partial\bm{q}_I}H^{ij}\beta_j\text{.}
\end{align}
Therefore, the remaining work is to calculate 
$\partial^2\alpha_i/\partial\bm{q}_J\partial\bm{q}_I$ and $\partial^2\beta_i/\partial\bm{q}_J\partial\bm{q}_I$.
The concrete form of the former can be easily deduced as
\begin{align}
  \frac{\partial^2\alpha_1}{\partial\bm{q}_J\partial\bm{q}_I}&=\varPhi^I_{,1}\varPhi^J_{,1}\bm{I}\text{,}\\
  \frac{\partial^2\alpha_2}{\partial\bm{q}_J\partial\bm{q}_I}&=\varPhi^I_{,2}\varPhi^J_{,2}\bm{I}\text{,}\\
  \frac{\partial^2\alpha_3}{\partial\bm{q}_J\partial\bm{q}_I}&=\left(\varPhi^I_{,1}\varPhi^J_{,2}+\varPhi^I_{,2}\varPhi^J_{,1}\right)\bm{I}\text{,}
\end{align}
while it takes some time to compute the latter, which satisfies
\begin{align}
  2\frac{\partial^2B_{\alpha\beta}}{\partial\bm{q}_J\partial\bm{q}_I}=&\frac{\partial^2b_{\alpha\beta}}{\partial\bm{q}_J\partial\bm{q}_I}\notag\\
  =&\varPhi^I_{,\alpha\beta}\frac{\partial\bm{a}_3}{\partial\bm{q}_J}+\varPhi^J_{,\alpha\beta}\left(\frac{\partial\bm{a}_3}{\partial\bm{q}_I}\right)^\mathrm{T}+\varPhi^I_{,1}\varPhi^J_{,1}\bm{D}^{11}\notag\\
  &+\varPhi^I_{,2}\varPhi^J_{,2}\bm{D}^{22}+\varPhi^I_{,1}\varPhi^J_{,2}\bm{D}^{12}+\varPhi^I_{,2}\varPhi^J_{,1}\bm{D}^{21}\text{,}
\end{align}
in which coefficients of the first-order terms are
\begin{align}
  \frac{\partial\bm{a}_3}{\partial\bm{q}_J}&=\frac{1}{\sqrt{a}}\left(-\varPhi^J_{,1}[\bm{a}_2]+\varPhi^J_{,2}[\bm{a}_1]-\bm{a}_3\otimes(\varPhi^J_{,1}\bm{t}_1+\varPhi^J_{,2}\bm{t}_2)\right)\text{,}\\
  \frac{\partial\bm{a}_3}{\partial\bm{q}_I}&=\frac{1}{\sqrt{a}}\left(-\varPhi^I_{,1}[\bm{a}_2]+\varPhi^I_{,2}[\bm{a}_1]-\bm{a}_3\otimes(\varPhi^I_{,1}\bm{t}_1+\varPhi^I_{,2}\bm{t}_2)\right)\text{,}
\end{align}
and coefficients of the second-order terms are respectively calculated by dot products of $\bm{a}_{\alpha,\beta}$ with $\partial^2\bm{a}_3/{\partial\bm{a}_1}^2$, $\partial^2\bm{a}_3/{\partial\bm{a}_2}^2$, ${\partial^2\bm{a}_3}/{\partial\bm{a}_2\partial\bm{a}_1}$, and ${\partial^2\bm{a}_3}/{\partial\bm{a}_1\partial\bm{a}_2}$.
For calculation, we provide relatively simple formulae as follows:
\begin{align}
  \bm{D}^{11}=&\frac{1}{a}\left(\beta_{\alpha\beta}(3\bm{t}_1\otimes\bm{t}_1+\bm{a}_2\otimes\bm{a}_2-a_{22}\bm{I})\right.\notag\\
  &\left.-\bm{s}_2\otimes\bm{t}_1-\bm{t}_1\otimes\bm{s}_2\right)\text{,}\\
  \bm{D}^{22}=&\frac{1}{a}\left(\beta_{\alpha\beta}(3\bm{t}_2\otimes\bm{t}_2+\bm{a}_1\otimes\bm{a}_1-a_{11}\bm{I})\right.\notag\\
  &\left.-\bm{s}_1\otimes\bm{t}_2-\bm{t}_2\otimes\bm{s}_1\right)\text{,}\\
  \bm{D}^{12}=&\frac{1}{a}\left(\beta_{\alpha\beta}(3\bm{t}_1\otimes\bm{t}_2-2\bm{a}_1\otimes\bm{a}_2+\bm{a}_2\otimes\bm{a}_1+a_{12}\bm{I})\right.\notag\\
  &\left.-\bm{s}_2\otimes\bm{t}_2-\bm{t}_1\otimes\bm{s}_1-\sqrt{a}[\bm{a}_{\alpha,\beta}]\right)\text{,}\\
  \bm{D}^{21}=&\frac{1}{a}\left(\beta_{\alpha\beta}(3\bm{t}_2\otimes\bm{t}_1-2\bm{a}_2\otimes\bm{a}_1+\bm{a}_1\otimes\bm{a}_2+a_{12}\bm{I})\right.\notag\\
  &\left.-\bm{s}_1\otimes\bm{t}_1-\bm{t}_2\otimes\bm{s}_2+\sqrt{a}[\bm{a}_{\alpha,\beta}]\right)\text{,}
\end{align}
where $t_1$, $t_2$, $s_1$, and $s_2$ are defined as
\begin{align}
  \bm{t}_1&=\bm{a}_2\times\bm{a}_3\text{,}\\
  \bm{t}_2&=\bm{a}_3\times\bm{a}_1\text{,}\\
  \bm{s}_1&=\bm{a}_{\alpha,\beta}\times\bm{a}_1\text{,}\\
  \bm{s}_2&=\bm{a}_2\times\bm{a}_{\alpha,\beta}\text{.}
\end{align}
Here we use $[\cdot]$ to represent the cross product matrix of a vector, which is defined as
\begin{equation}
  \left[\begin{pmatrix}v_1\\v_2\\v_3\end{pmatrix}\right]=
  \begin{pmatrix}
    0&-v_3&v_2\\
    v_3&0&-v_1\\
    -v_2&v_1&0
  \end{pmatrix}
  \text{.}
\end{equation}

\paragraph{The pseudo Hessian}
In the calculation of the Hessian matrix, the term $\partial^2\beta_i/\partial\bm{q}_J\partial\bm{q}_I$ takes up the most time.
Thanks to the low magnitude of this term, we can subtract it to construct an inexact Hessian matrix, which significantly reduces the time consumption per step.
Note that an inexact Hessian in general shows better positiveness than its exact version, and thus it may also reduce the number of iterations in certain cases.

==> src_sup/mathematics.tex <==
\section{Mathematical tools}

\subsection{Bicubic Hermite Interpolation}
\label{apx:hermite}

Thoroughly, the midsurface in BHEM is parameterized by
\begin{equation}
  \label{eqn:hermite}
  \bm{x}(\xi^1,\xi^2)=\sum_{p,q,r,s\in\{0,1\}}w_{pq,rs}(\theta^1,\theta^2)\bm{x}_{pq,rs}\text{,}
\end{equation}
in which $\bm{x}_{pq,rs}$ represents $4$ generalized coordinates of node $\bm{x}_{pq}$, with $r$ and $s$ denoting the order of partial derivatives w.r.t. $\xi^1$ and $\xi^2$, respectively. See Fig.~5 of the main text.
The weight function $w_{pq,rs}$ takes the form of
\begin{equation}
  w_{pq,rs}(\theta^1,\theta^2)=w_{p,r}(\theta^1)\,w_{q,s}(\theta^2)\text{,}
  \label{eqn:hermite_weight}
\end{equation}
with $\theta^\alpha\in[0,1]$ defined as $(\xi^\alpha-\xi_\mathrm{min}^\alpha)/\Delta\xi^\alpha$.

As written in Eq.~(\ref{eqn:hermite_weight}), bicubic Hermite interpolation indicates using a cubic basis function in each dimension of the parameter space.
To be specific, $w_{p,r}$ is defined as follows:
\begin{subnumcases}{w_{p,r}(\theta)=}
  f(\theta)\text{,}&$p=0\land r=0$,\\
  f(1-\theta)\text{,}&$p=1\land r=0$,\\
  g(\theta)\text{,}&$p=0\land r=1$,\\
  -g(1-\theta)\text{,}&$p=1\land r=1$,
\end{subnumcases}
where $f(\theta)=2\theta^3-3\theta^2+1$ and $g(\theta)=\theta^3-2\theta^2+\theta$ hold. $w_{q,s}$ is defined similarly by replacing indices.

Furthermore, taking the derivative of Eq.~(\ref{eqn:hermite}) yields
\begin{align}
  \bm{a}_1(\xi^1,\xi^2)&=\sum_{p,q,r,s\in\{0,1\}}\frac{1}{\Delta\xi^1}w'_{p,r}(\theta^1)\,w_{q,s}(\theta^2)\,\bm{x}_{pq,rs}\text{,}\\
  \bm{a}_2(\xi^1,\xi^2)&=\sum_{p,q,r,s\in\{0,1\}}\frac{1}{\Delta\xi^2}w_{p,r}(\theta^1)\,w'_{q,s}(\theta^2)\,\bm{x}_{pq,rs}\text{,}
\end{align}
where
\begin{subnumcases}{w'_{p,r}(\theta)=}
  f'(\theta)\text{,}&$p=0\land r=0$,\\
  -f'(1-\theta)\text{,}&$p=1\land r=0$,\\
  g'(\theta)\text{,}&$p=0\land r=1$,\\
  g'(1-\theta)\text{,}&$p=1\land r=1$,
\end{subnumcases}
with $f'(\theta)=6\theta^2-6\theta$ and $g'(\theta)=3\theta^2-4\theta+1$ holding. $w'_{q,s}(\theta)$ can be still formalized by replacing indices.

It is clear that all the following equations hold: $f(0)=1$, $f(1)=0$, $g(0)=0$, $g(1)=0$, $f'(0)=0$, $f'(1)=0$, $g'(0)=1$, and $g'(1)=0$, which means that the values of $\bm{x}$, $\bm{a}_1$, and $\bm{a}_2$ on a common edge are merely related to the sampled values at the two end nodes of the edge. This implies $\mathcal{C}^1$-smoothness on the whole surface --- the interpolation function itself and its first-order partial derivatives remain continuous across cells, while the second-order partial derivatives come to discontinuity of first kind only at the common edges.

\subsection{Gauss--Legendre Quadrature}
\label{apx:quadrature}

\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=0.5]
    \draw[step=4] (0,0) grid (4,4);
    \tikzmath{\xa=0.339981;};
    \tikzmath{\xb=0.861136;};
    \tikzmath{\ta=2-\xb*2;};
    \tikzmath{\tb=2-\xa*2;};
    \tikzmath{\tc=2+\xa*2;};
    \tikzmath{\td=2+\xb*2;};
    \foreach \x in {\ta,\tb,\tc,\td}{
      \foreach \y in {\ta,\tb,\tc,\td}{
        \fill (\x,\y) circle (0.06667);
      }
      \draw[dashed] (\x,0)--(\x,4);
      \draw[dashed] (0,\x)--(4,\x);
    }
\end{tikzpicture}
\caption{Quadrature points in a cell.}
\label{fig:quadrature}
\vspace{-0.3cm}
\end{figure}

Any two-dimensional integral that takes the form of
\begin{equation}
  I=
  \int_{\xi_\mathrm{min}^2}^{\xi_\mathrm{max}^2}
  \int_{\xi_\mathrm{min}^1}^{\xi_\mathrm{max}^1}
  f(\xi^1,\xi^2)\,\mathrm{d}\xi^1\mathrm{d}\xi^2\text{,}
\end{equation}
can be computed approximately using the summation of $n$ sampled points that
\begin{equation}
  I\approx\sum_{i=1}^{n}w_if(\xi^1_i,\xi^2_i)\text{.}
\end{equation}
We pick $n=16$ in our framework, with the quadrature points arranged by $4\times4$ in a single cell. As shown in Fig.~\ref{fig:quadrature}, the vertical dashed lines correspond to
\begin{equation}
  \theta^1=\frac{\xi_\mathrm{min}^1+\xi_\mathrm{max}^1}{2}\pm\frac{\Delta\xi^1}{2}\sqrt{\frac{3}{7}\pm\frac{2}{7}\sqrt{\frac{6}{5}}}\text{,}
\end{equation}
respectively, and the horizontal dashed lines correspond to 
\begin{equation}
  \theta^2=\frac{\xi_\mathrm{min}^2+\xi_\mathrm{max}^2}{2}\pm\frac{\Delta\xi^2}{2}\sqrt{\frac{3}{7}\pm\frac{2}{7}\sqrt{\frac{6}{5}}}\text{,}
\end{equation}
respectively. The inside vertical lines equip a weight factor of $(18+\sqrt{30})\Delta\xi^1/72$, while the outside ones equip a weight factor of $(18-\sqrt{30})\Delta\xi^1/72$. The inside horizontal lines equip a weight factor of $(18+\sqrt{30})\Delta\xi^2/72$, while the outside ones equip a weight factor of $(18-\sqrt{30})\Delta\xi^2/72$. The final weight $w_i$ of each point is the product of the two weights of the vertical and horizontal lines it lies on.


==> src_sup/notation.tex <==
%!TEX root = ../main.tex

\newcommand{\name}{RainyGS}
\newcommand{\gs}{Gaussian Splatting}
\newcommand{\gsshort}{3DGS}
% general scalars
\newcommand{\qy}[1]{{\color{Green}{#1}}}
\newcommand{\xy}[1]{{\color{Orange}{#1}}}
\newcommand{\wz}[1]{{\color{Red}{wz:#1}}}

\newcommand{\methodshort}{{4DGS}}
\newcommand{\method}{{4D Gaussian Splatting}}
\newcommand{\methodgaussiansplattingshort}{{3DGS}}
\newcommand{\methodgaussiantrackingshort}{{Dyanmic-3DG}}
\newcommand{\methodiclrshort}{{4DGS-Y}}
\newcommand{\methodsplit}{{scale-split}}
\newcommand{\gshader}{{GaussianShader}}
\newcommand{\gof}{{Gaussian Opacity Fields}}
\newcommand{\gofshort}{{GOF}}
\newcommand{\gshadershort}{{GShader}}


% change this value in a section to use/override draft mode for figures
\newcommand{\hidesectionfigures}{false}

% highlighting changes by various authors
%\newcommand{\changeK}[1]{{\added{#1}}}
%\newcommand{\changeP}[1]{{\added{#1}}}
%\newcommand{\changeW}[1]{{\added{#1}}}

%\newcommand{\addP}[1]{\added[id=P]{#1}}
% add id if you want the author name to appear 
% as a superscript
%\newcommand{\addP}[1]{{\color{blue}{#1}}}
\newcommand{\addP}[1]{\added{#1}}
\newcommand{\deleteP}[1]{\deleted{#1}}
\newcommand{\replaceP}[2]{\replaced{#1}{#2}}

% use the following versions if you want the author name to appear 
% as a superscript
%\newcommand{\changeK}[1]{{\color{red}{#1}}}	
\newcommand{\changeK}[1]{{{#1}}}		
\newcommand{\changeP}[1]{{\added[id=P]{#1}}}
\newcommand{\changeW}[1]{{\added[id=W]{#1}}}

\newcommand{\penaltyName}{penalty\xspace}

%% decoders
\newcommand{\znccneigh}[1]{ZNCC$_{#1}$}
\newcommand{\znccneighnn}[1]{ZNCC-NN$_{#1}$}
		

%% punctuation for equations
\newcommand{\eqcomma}{\ \ ,}
\newcommand{\eqstop}{\ \ .}

% math

% current
\newcommand{\curView}{V}
\newcommand{\rgbSrc}{I_s}
\newcommand{\depthMap}{D}
\newcommand{\normalMap}{N}
\newcommand{\heightMap}{H}
\newcommand{\semMask}{H}
%


\newcommand{\threeDGaussian}{G}
\newcommand{\point}{\bm{x}}
\newcommand{\centerPos}{\bm{\mu}}
\newcommand{\threeDCov}{\bm{\Sigma}}
\newcommand{\threeDScaling}{\bm{S}}
\newcommand{\threeDRotation}{\bm{R}}
\newcommand{\threeDPosition}{\bm{x}}
\newcommand{\opacity}{o}
\newcommand{\twoDCov}{\bm{\Sigma}'}
\newcommand{\Jacobian}{\bm{J}}
\newcommand{\extrinsic}{\bm{V}}
\newcommand{\twoDGaussianFromThreeDG}{G'}
\newcommand{\pixelColor}{C}
\newcommand{\weightBlending}{\alpha}

\newcommand{\fourDGaussian}{G_{4D}}
\newcommand{\fourDCenter}{\mu_{4D}}
\newcommand{\fourDCov}{\Sigma_{4D}}
\newcommand{\fourDScaling}{S_{4D}}
\newcommand{\fourDRotation}{R_{4D}}

\newcommand{\rotorFour}{r}
\newcommand{\rotorFourCoef}{r_c}
\newcommand{\s}{s}
\newcommand{\bi}{b}
% \newcommand{\bZeroOne}{b_{01}}
% \newcommand{\bZeroTwo}{b_{02}}
% \newcommand{\bZeroThree}{b_{03}}
% \newcommand{\bOneTwo}{b_{12}}
% \newcommand{\bOneThree}{b_{13}}
% \newcommand{\bTwoThree}{b_{23}}
\newcommand{\p}{p}
\newcommand{\e}{e}
% \newcommand{\eZeroOne}{e_{01}}
% \newcommand{\eZeroTwo}{e_{02}}
% \newcommand{\eZeroThree}{e_{03}}
% \newcommand{\eOneTwo}{e_{12}}
% \newcommand{\eOneThree}{e_{13}}
% \newcommand{\eTwoThree}{e_{23}}
% \newcommand{\eOneTwoThreeFour}{e_{0123}}

\newcommand{\deltA}{\delta}
\newcommand{\length}{l}
\newcommand{\varepsiloN}{\varepsilon}
\newcommand{\DeltA}{\Delta}
\newcommand{\uSrcFourD}{u}
\newcommand{\uTargetFourD}{u'}

\newcommand{\threeDGaussianFromFourDG}{G_{3D}}
\newcommand{\threeDCovFromfourDCov}{\Sigma_{3D}}
\newcommand{\U}{U}
\newcommand{\V}{V}
\newcommand{\W}{W}
\newcommand{\A}{A}
\newcommand{\M}{M}
\newcommand{\Z}{Z}
\newcommand{\lambdA}{\lambda}
\newcommand{\timeT}{t}

\newcommand{\loss}{L}
\newcommand{\depth}{d}

\newcommand{\del}{\bm{\nabla}}
